Learning Sentence-internal Temporal Relations

In this paper we propose a data intensive approach for inferring sentence-internal temporal relations. Temporal inference is relevant for practical NLP applications which either extract or synthesize temporal information (e.g., summarisation, question answering). Our method bypasses the need for manual coding by exploiting the presence of markers like after", which overtly signal a temporal relation. We first show that models trained on main and subordinate clauses connected with a temporal marker achieve good performance on a pseudo-disambiguation task simulating temporal inference (during testing the temporal marker is treated as unseen and the models must select the right marker from a set of possible candidates). Secondly, we assess whether the proposed approach holds promise for the semi-automatic creation of temporal annotations. Specifically, we use a model trained on noisy and approximate data (i.e., main and subordinate clauses) to predict intra-sentential relations present in TimeBank, a corpus annotated rich temporal information. Our experiments compare and contrast several probabilistic models differing in their feature space, linguistic assumptions and data requirements. We evaluate performance against gold standard corpora and also against human subjects.

==> jairfiles/authors-guide <==

  		 Instructions for Final preparation 
		              Author's guide 


INSTRUCTIONS FOR FINAL PREPARATION: AUTHOR'S GUIDE

This file is available via our FTP server at CMU:

CMU Machine:   ftp.cs.cmu.edu  
       file: /project/jair/information/format/authors-guide

-----------------------------------------------------------------
Checklist (see detailed instructions below)

1. [ ] Format article using JAIR style
2. [ ] Have your article proofread.
3. [ ] Create HTML version (strongly recommended, but not required)
4. [ ] Contact editor, obtain final approval
5. [ ] Contact Steven Minton, Managing Editor, (minton@isi.edu) for formatting check
6. [ ] Final changes on HTML, online appendices, etc.
7. [ ] Fill out copyright transfer, and send it.
8. [ ] Fill out source code release, and sent it (only necessary if you are releasing source 
         code in an online appendix).
9. [ ] Contact Managing Editor (minton@fetch.com) for page numbers, then send all the 
         required files.
10.[ ] Also inform Managing Editor of any special mailing lists or newsgroups you'd 
         like an announcement sent to.
11.[ ] After your article is published, create forward pointers (optional)
       
-----------------------------------------------------------------------

Once a paper has been accepted for publication in JAIR, you should follow the procedure 
outlined below. The final version of your manuscript is due to us *within three months* 
of the acceptance date. If you require more than three months, please request an extension 
from the editor. 

1. Format your article according the JAIR style, which is described in format.ps and the other 
files in the directory information/format. There are subdirectories for LaTex, FrameMaker 
and Gnu's GROFF. (We request that you use LaTex if possible.)  Authors are responsible 
for correctly formatting their article. If you wish we can recommend professionals who will 
do this for you for a fee.

Here are things to check, *before* you send us your article:
   - Capitalize section and subsection titles.
   - Make sure your abstract reads well. It will be used to advertise your paper.
   - We recommend you use small caps for system names. (In LaTex that's \sc) 
   - Capitalize references to figures and tables, e.g. "In Figure 7..."
   - It's preferable to cite published papers, rather than tech reports.
   - Carefully read the section on citations in format.ps. Here are examples of BAD citations:
        "See (Ginsberg, 1994) for an analysis..." 
                 [Uses citation as a noun] 
        "Drummond (Drummond, 1994) showed that..." 
                 [Should use citeyear i.e., Drummond (1994)] 
        "...the best method (see the ERT test (Davis, 1995))..." 
                 [double parens, should be  
        "...best method (see the ERT test, Davis, 1995)..."] 
   - In the authors' addresses, don't use commas at the end of the lines.
- Do not start a section with a subsection. (E.g., Each section should start with some text, 
   rather than immediately starting with a subsection.) Similarly, don't start a subsection 
   with a sub-subsection.
- Your paper should be formatted for 8.5 x 11 letter size paper, not A4 (common in Europe). 
   If you are in Europe and use Latex, use "dvips -t" when you create your PostScript file to 
   get the right size.

2. Make any final changes and have your article proofread. For better or worse, we do not 
have a copyediting staff. (Note: Authors are notoriously bad proofreaders. Have the paper 
proofread by a skilled proofreader -- NOT one of the authors.)

3. JAIR offers authors  the option of publishing a version of the paper in  HTML in 
addition to the PostScript version. Check out the Latex2HTML translator at the 
following URL: http://cbl.leeds.ac.uk/nikos/tex2html/doc/latex2html/latex2html.html (If you 
use Latex2HTML, don't bother using the JAIR style file, as it will only cause problems.)

We also encourage you to make use of "online appendices" where appropriate. Online 
appendices can contain source code, data, even quicktime demonstrations -- anything that 
will make life easier (or more interesting) for your readers and researchers who follow in your 
footsteps.

4. Send the paper to the editor in charge of your article. Also send a copy to jair-ed@isi.edu.

5. Once the editor approves the paper, he or she will tell you to send a copy of the PostScript 
file to the managing editor, Steven Minton, minton@fetch.com. He will check it over quickly, and 
if the formatting is acceptable, we will let you know the publication date and the page numbers 
for your article.

6. Once you have the final approval on the paper and the formatting you should put the final 
touches on any additional versions of the paper that you want us to publish alongside the 
PostScript version. As noted above, we encourage authors to produce an HTML version of 
their paper.

7. Please print out, fill in, and sign the Postscript Transfer of Copyright form in this directory. 
(If you have trouble printing the PostScript, we can send you an ascii version.)
Send the form to:
     Steven Minton
     Fetch Technologies
     2041 Rosecrans Avenue, Suite 245
     El Segundo, CA 90245-4789

The copyright transfer is necessary because it's part of our agreement with AAAI Press .  
Once you transfer the copyright, AI Access Foundation grants the rights to publish 
the hardcopy version to AAAI Press. But because AI Access Foundation wants to 
promote the widest possible distribution of your article, we are happy to grant you back any 
other rights  you want to the article or the contents. In particular, the electronic version is freely 
available for distribution -- that's part of our mission.

8. If there are online appendices containing source code, please sign the release form found in 
this directory and send it along with the Transfer of Copyright. The release form is intended 
to reduce the liability of AI Access Foundation and JAIR's distributors.

9. Once the managing editor (minton@isi.edu) approves the formatting and sends you the 
publication date and page numbers, please send him all the files. (A single tar file is convenient.) 
We would appreciate it if you use the following naming scheme for your files. Assuming the 
first author's last name is "Jones" and the current year is 1999, you should send us:
   - jones99a.ps, the final PostScript file
   - jones99a.tex (or jones99a.txt), a single LaTex source file (or, if you didn't use LaTex, some sort 
     of ascii version of the paper if possible) which we can use for our search engine
   - jones99a.tar, a tar file containing all the source files (latex files, figures, word file, whatever) 
     which we will archive. 
   - [optional] jones99a.pdf, a PDF version of your paper. We will create one ourselves if you don't 
      send it to us.
   - [optional] jones99a-html.tar, a tar file of a directory called jones99a-html containing the HTML 
      version of your paper.
   - [optional] jones99a-appendix1.txt (or .ps, .lisp, or .whatever), an online appendix. If there are 
      two or more, name them jones99a-appendix2.txt and so on.

Note: in the unlikely case that the first author has a previously published a JAIR article earlier in 
the year called jones99a, use jones99b this time.

As an alternative to emailing the files, you can send FTP instructions to the managing editor.

10. After we receive the final version and release the article, we will post an announcement on 
the JAIR newgroup comp.ai.jair.announcments.  We send out regular announcements 
to our mailing list for people that don't read netnews.  If you know of any other mailing lists where it 
would be appropriate to post an announcement for your paper (e.g. ML-LIST for machine 
learning papers), please feel free to forward our announcement. 


11. After your article is published, you can create an HTML page listing pointers to subsequent 
papers you (or others, if you wish) write on the same topic.  JAIR will maintain a pointer to this 
page, assuming you agree to maintain the page of forward pointers. Contact the Managing Editor 
if you are interested in this.

Congratulations!



